Generative Pre-training for Paraphrase Generation by Representing and Predicting Spans in Exemplars

Paraphrase generation is a long-standing problem and serves an essential role in many natural language processing problems. Despite some encouraging results, recent methods either confront the problem of favoring generic utterance or need to retrain the model from scratch for each new dataset. This paper presents a novel approach to paraphrasing sentences, extended from the GPT-2 model. We develop a template masking technique, named first-order masking, to masked out irrelevant words in exemplars utilizing POS taggers. So that, the paraphrasing task is changed to predicting spans in masked templates. Our proposed approach outperforms competitive baselines, especially in the semantic preservation aspect. To prevent the model from being biased towards a given template, we introduce a technique, referred to as second-order masking, which utilizes Bernoulli distribution to control the visibility of the first-order-masked template's tokens. Moreover, this technique allows the model to provide various paraphrased sentences in testing by adjusting the second-order-masking level. For scale-up objectives, we compare the performance of two alternatives template-selection methods, which shows that they were equivalent in preserving semantic information.

==> tables/baseline_compare2_old.tex <==
\begin{table*}[htbp] 
    \centering
    \caption{Results on the QQP-Pos and ParaNMT-small dataset. In all metrics, a higher score is better. ParafraGPT-U is trained on lowercased pre-processed datasets as similar to SGCP, whereas ParafraGPT-C runs on the case-sensitive version. ParafraGPT-UC handles both types of data, which is trained a half of time for each one. Specifically, Source-as-Output and Exemplar-as-Output are used only for indicator purposes }
    \begin{center}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{lcccccccccc}
            \hline
                &\multicolumn{5}{c}{QQP-Pos}&\multicolumn{5}{c}{ParaNMT-small} \\
            \hline
             Models & BLEU & ROUGE-1 & ROUGE-2 & ROUGE-L & BERT SCORE & BLEU & ROUGE-1 & ROUGE-2 & ROUGE-L & BERT SCORE\\
             \hline
             Source-as-Output & 17.2 & 51.9 & 26.2 & 52.9 & 84.9 & 18.5 & 50.6 & 23.1 & 47.7 & 86.2\\
            Exemplar-as-Output & 16.8 & 38.2 & 20.5 & 43.2 & 78.2  & 3.3 & 24.4 & 7.5 & 29.1 & 74.2\\
            \hline
            SCPN \cite{iyyer2018adversarial} & 15.6 & 40.6 & 20.5 & 44.6 & -  & 6.4 & 30.3 & 11.2 & 34.6 & -\\
            CGEN \cite{chen2019controllable} & 34.9 & 62.6 & \underline{42.7} & 65.4 & -  & 13.6 & 44.8 & 21.0 & \textbf{48.3} & -\\
            SGCP \cite{kumar2020syntax} & \textbf{36.7} & \underline{66.9} & \textbf{45.0} & \textbf{69.6} & 85.7  & 15.3 & \underline{46.6} & \textbf{21.8} & \textbf{49.7} & 80.5\\
            \hline 
            GPT-2-small & 16.1 & 54.5 & 23.5 & 49.8 & 84.5 & 7.3 & 44.3 & 14.8 & 39.8 & \underline{80.7} \\
            \hline
            ParafraGPT-U & 34.7 & 66.5 & 40.3 & 65.1 & \underline{86.6} & \underline{15.2} & \textbf{49.2} & \underline{21.4} & 46.2 & \textbf{82.4}\\
            ParafraGPT-C & 35.5 & 66.6 & 40.7 & 65.5 & \textbf{89.2}  & - & - & - & - & -\\
            ParafraGPT-UC & \underline{35.6} & \textbf{67.1} & 41.5 & \underline{65.8} & \textbf{89.2}  & - & - & - & - & -\\
            \hline 
        \end{tabular}
        }
    \end{center}
    \label{tbl:comparison_baselines}
\end{table*}


==> tables/baseline_comparison.tex <==
\begin{table*}[htbp] 
    \centering
    \caption{Comparision about \textit{mpA}, the number of parameters, model training time between existing gradient based method(\textit{TfS}, \textit{LwF}) and our non-gradient based attention method(\textit{NGbA}) on \textit{VoxCeleb2}.}
    \begin{center}
        \resizebox{\textwidth}{!}{
        \begin{tabular}{ccccccc}
            \hline
                \multicolumn{7}{c}{QQPPos} \\
            \hline
             Model & BLEU & METEOR & ROUGE-1 & ROUGE-2 & ROUGE-L & BERT SCORE \\
             \hline
             Source-as-Output (Processed) & 17.2 & 31.1 & 51.9 & 26.2 & 52.9 & 84.9\\
             Exemplar-as-Output (Processed) & 16.8 & 17.6 & 38.2 & 20.5 & 43.2 & 78.2 \\
             Source-as-Output (Original) & & & & & & 85.9\\
             Exemplar-as-Output (Original) & & & & & & 77.8\\
            \hline
            SCPN & 15.6 & 19.6 & 40.6 & 20.5 & 44.6 & - \\
            CGEN & 34.9 & 37.4 & 62.6 & 42.7 & 65.4 & - \\
            SGCP & 36.7 & 39.8 & 66.9 & 45.0 & 69.6 & 85.7 \\
            \hline 
            GPT2 & 27.8 & & & & & 85.5\\
            Uncased-Exemplar GPT2 & 33.7 & 39.1 & 66.5 & 40.3 & 65.1 & 86.6\\
            Uncased-Cased-Exemplar GPT2 & 35.6 & 39.9 & 67.1 & 41.5 & 65.8 & 89.2 \\
            Cased-Exemplar GPT2 & 35.5 & 39.5 & 66.6 & 40.7 & 65.5 & 89.2 \\
            \hline 
            \multicolumn{7}{c}{ParaNMT-small} \\
            \hline
            Source-as-Output (Processed) & 18.5 & 28.8 & 50.6 & 23.1 & 47.7 & 86.2 \\
            Exemplar-as-Output (Processed) & 3.3 & 12.1 & 24.4 & 7.5 & 29.1 & 74.2 \\ 
            \hline
            SCPN & 6.4 & 14.6 & 30.3 & 11.2 & 34.6 & - \\
            CGEN & 13.6 & 24.8 & 44.8 & 21.0 & 48.3 & - \\
            SGCP & 15.3 & 25.9 & 46.6 & 21.8 & 49.7 & 81.2 \\
            \hline
            GPT2 & \\
            Uncased-Exemplar GPT2 & 15.4 & 26.4 & 49.2 & 21.4 & 46.2 & 82.4 \\
            Uncased-Cased-Exemplar GPT2 & 14.8 & & 49.2 & 21.4 & 46.2 & 82.4 \\
            Cased-Exemplar GPT2 & 14.8 & & 49.2 & 21.4 & 46.2 & 82.4 \\
            \hline
        \end{tabular}
        }
    \end{center}
    \label{table:exp_3_voxceleb2}
\end{table*}


==> tables/partly_training.tex <==
\begin{table}[htbp] 
    \centering
    \caption{Results on partial fine-tuning the pre-trained model. }
    \begin{center}
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{lccccc}
            \hline
             Fine-tuning methods& BLEU & ROUGE-1 & ROUGE-2 & ROUGE-L & BERT SCORE \\
            %  1.31 | 1.13 | 1.26
            \hline
            All parameters & 35.6 & 66.1 & 43.5 & 68.3 & 88.9 \\
            Embed, pred, last & 28.8 & 61.4 & 36.6 & 63.6 & 86.2 \\ 
            Gradual unfreezing & 28.0 & 61.3 & 35.4 & 63.1 & 86.1\\ 
            \hline 
        \end{tabular}
        }
    \end{center}
    \label{tbl:partial_training}
\end{table}


==> tables/tgt_mask.tex <==
\begin{table}[htbp] 
    \centering
    \caption{Results on template selection methods. We compare the performance of TED-based template selection with the embedding-based one.}
    \begin{center}
        \resizebox{\columnwidth}{!}{
        \begin{tabular}{lccccc}
            \hline
             P & BLEU & ROUGE-1 & ROUGE-2 & ROUGE-L & BERT SCORE \\
            \hline
            0.0 & 35.6 & 66.1 & 43.5 & 68.3 & 88.5 \\ 
            0.05 & 35.8 & 66.2 & 43.7 & 68.4 & 88.5 \\ 
            0.1 & 35.6 & 66.2 & 43.5 & 68.4 & 88.4 \\ 
            0.15 & 35.4 & 66.1 & 43.4 & 68.3 & 88.4 \\ 
            0.20 & 35.3 & 65.9 & 43.4 & 68.1 & 88.4 \\ 
            0.25 & 34.7 & 65.7 & 42.8 & 67.9 & 88.3 \\ 
            0.30 & 34.0 & 65.4 & 42.0 & 67.5 & 88.2 \\ 
            0.35 & 33.4 & 65.2 & 41.4 & 67.3 & 88.1 \\ 
            0.40 & 32.8 & 64.9 & 41.0 & 66.9 & 88.0 \\ 
            0.45 & 31.8 & 64.1 & 40.0 & 66.1 & 87.8 \\ 
            0.50 & 30.9 & 63.4 & 39.1 & 65.5 & 87.6 \\ 
            0.55 & 30.1 & 63.1 & 38.5 & 65.1 & 87.4 \\ 
            0.60 & 29.1 & 62.5 & 37.6 & 64.4 & 87.2 \\ 
            0.65 & 28.3 & 62.0 & 37.0 & 63.9 & 87.1 \\ 
            0.70 & 27.2 & 61.0 & 35.9 & 62.9 & 86.9 \\ 
            0.75 & 25.9 & 60.1 & 34.7 & 62.0 & 86.6 \\ 
            0.80 & 24.3 & 58.9 & 33.2 & 60.7 & 86.3 \\ 
            0.85 & 22.5 & 57.5 & 31.6 & 59.3 & 86.0 \\ 
            0.90 & 21.2 & 56.1 & 30.4 & 57.9 & 85.7 \\ 
            0.95 & 19.6 & 54.8 & 29.0 & 56.6 & 85.4 \\ 
            1.0 & 17.5 & 53.2 & 27.3 & 54.9 & 85.0 \\ 
            
            \hline 
        \end{tabular}
        }
    \end{center}
    \label{tbl:template_compare}
\end{table}


==> tables/tokens.tex <==
\begin{table}[ht]
    \centering
    \caption{List of additional tokens to ParafraGPT}
    \begin{tabular}{c|l}
         Token & Role \\
         \hline
         \<sos\> & Start of sequence \\
         \<eos\> & End of sequence \\
         \<sep\> & Separate a source and a template \\
         \<eq\>  & Separate a source-template pair and a target
    \end{tabular}
    
    \label{tbl:tokens}
\end{table}
